QUIJOTE scientific results -- IV. A northern sky survey in intensity and polarization at 10-20GHz with the Multi-Frequency Instrument

We present QUIJOTE intensity and polarization maps in four frequency bands centred around 11, 13, 17 and 19GHz, and covering approximately 29000 deg$^2$, including most of the Northern sky region. These maps result from 9000 h of observations taken between May 2013 and June 2018 with the first QUIJOTE instrument (MFI), and have angular resolutions of around $1^\circ$, and sensitivities in polarization within the range 35-40 $\mu$K per 1-degree beam, being a factor $\sim 2$-$4$ worse in intensity. We discuss the data processing pipeline employed, and the basic characteristics of the maps in terms of real space statistics and angular power spectra. A number of validation tests have been applied to characterise the accuracy of the calibration and the residual level of systematic effects, finding a conservative overall calibration uncertainty of 5%. We also discuss flux densities for four bright celestial sources (Tau A, Cas A, Cyg A and 3C274) which are often used as calibrators at microwave frequencies. The polarization signal in our maps is dominated by synchrotron emission. The distribution of spectral index values between the 11GHz and WMAP 23GHz map peaks at $\beta=-3.09$ with a standard deviation of 0.14. The measured BB/EE ratio at scales of $\ell=80$ is $0.26\pm 0.07$ for a Galactic cut $|b|>10^\circ$. We find a positive TE correlation for 11GHz at large angular scales ($\ell \lesssim 50$), while the EB and TB signals are consistent with zero in the multipole range $30 \lesssim \ell \lesssim 150$. The maps discussed in this paper are publicly available.

==> table6_fit2noisespectrum_nochi2_commonbaselines.tex <==

\begin{table}
\caption{Noise levels from the fit to the noise power spectra based on
  the parametric equation~\ref{eq:fit_cl}, computed from the
  half-mission null tests with common baselines. In polarization, we show the results of the
fit to the EE spectra. Results for BB are fully consistent. }
\label{tab:noiseps2}
\centering
\begin{tabular}{@{}ccccc}
\hline
Channel & $C_{\rm w}$ & $\sigmadeg$ & $\alpha$ & $\ell_{\rm k}$ \\
 & [mK$^2$\,sr] & [$\mu$K] & &  \\
\hline
\multicolumn{5}{c}{Intensity (TT)}\\
\hline
217 & $5.82\times 10^{-6}$ & 130.0 & 0.94 & 239.8  \\
219 & $9.94\times 10^{-6}$ & 169.0 & 1.19 & 254.9  \\
311 & $2.43\times 10^{-6}$ &  84.1 & 0.83 & 219.4  \\
313 & $1.24\times 10^{-6}$ &  60.0 & 1.02 & 209.5  \\
417 & $1.03\times 10^{-5}$ & 172.7 & 0.92 & 281.0  \\
419 & $1.33\times 10^{-5}$ & 196.6 & 1.16 & 289.2  \\
\hline
\multicolumn{5}{c}{Polarization (EE)}\\
\hline
217 & $1.18\times 10^{-6}$ & 58.5 & 1.07 & 115.0  \\
219 & $1.81\times 10^{-6}$ & 72.5 & 1.16 & 147.7  \\
311 & $5.95\times 10^{-7}$ & 41.6 & 0.91 & 57.3  \\
313 & $4.83\times 10^{-7}$ & 37.5 & 1.10 & 53.4  \\
417 & $4.31\times 10^{-7}$ & 35.4 & 0.66 & 18.5  \\
419 & $4.88\times 10^{-7}$ & 37.6 & 0.76 & 33.9  \\
\hline
\end{tabular}
\end{table}


